Accelerating auxiliary-field quantum Monte Carlo with mixed-precision random propagators

We develop an algorithm to propagate auxiliary-field quantum Monte Carlo (AFQMC) wavefunctions in mixed precision. We target NVIDIA Tensor Cores using the TensorFloat-32 (TF32) format. We approximate each full-precision array by a TF32 leading term and a TF32 residual, and each full-precision matrix product by three TF32 products accumulated in full precision. Benchmarks on hydrogen chains show that mixed-precision propagation is consistently faster than double-precision GPU propagation, with an increasing advantage as the system size grows. The resulting local-energy deviations remain small over the propagation windows considered here. These results identify the stochastic two-body propagator as a particularly effective target for reduced precision, while our method allows higher precision to be retained for accuracy-sensitive operations. Hence, our algorithm provides a practical way to speed up AFQMC calculations and demonstrates where reduced precision can be applied without adverse effects on the method's accuracy.

==> command.tex <==

% Text
\newcommand{\supt}[1]{\textsuperscript{#1}}
\newcommand{\subt}[1]{\textsubscript{#1}}

% Math
\newcommand{\expn}[1]{\ {\operatorname{exp}}\left[{#1}\right]}

% Matrix elements
\newcommand{\h}[2]{{h}_{#1}^{#2}} % one-electron integrals
\renewcommand{\v}[2]{{v}_{#1}^{#2}} % two-electron integrals
\newcommand{\qh}[2]{{\tilde{h}}_{#1}^{#2}} % QED one-electron integrals
\newcommand{\qv}[2]{{\tilde{v}}_{#1}^{#2}} % QED two-electron integrals
\newcommand{\dm}[2]{{\rho}_{#1}^{#2}} % electronic density matrix
\newcommand{\f}[2]{{f}_{#1}^{#2}} % Fock matrix
\renewcommand{\d}[2]{{\delta}_{#1}^{#2}} % Kronecker delta

% Boson/fermion annihilation and creation operators
\newcommand{\ab}[1]{{\hat{b}}_{#1}^{}}
\newcommand{\cb}[1]{{\hat{b}}_{#1}^{\dagger}}
\newcommand{\af}[1]{{\hat{a}}_{#1}^{}}
\newcommand{\cf}[1]{{\hat{a}}_{#1}^{\dagger}}

% Symbols
\newcommand{\al}{\alpha}
\newcommand{\Ga}{\Gamma}
\newcommand{\ga}{\gamma}
\newcommand{\de}{\delta}
\newcommand{\om}{\omega}
\newcommand{\sg}{\sigma}
\newcommand{\la}{\lambda}
\newcommand{\ra}{\rightarrow}

% Bold letters
\newcommand{\bB}{\boldsymbol{B}}
\newcommand{\bD}{\boldsymbol{D}}
\newcommand{\bd}{\boldsymbol{d}}
\newcommand{\be}{\boldsymbol{e}}
\newcommand{\bG}{\boldsymbol{G}}
\newcommand{\bg}{\boldsymbol{g}}
\newcommand{\bn}{\boldsymbol{n}}
\newcommand{\bQ}{\boldsymbol{Q}}
\newcommand{\bq}{\boldsymbol{q}}
\newcommand{\bR}{\boldsymbol{R}}
\newcommand{\br}{\boldsymbol{r}}
\newcommand{\bU}{\boldsymbol{U}}
\newcommand{\bz}{\boldsymbol{z}}

% Bold symbols
\newcommand{\bet}{\boldsymbol{\eta}}
\newcommand{\bla}{\boldsymbol{\lambda}}
\newcommand{\bmu}{\boldsymbol{\mu}}

% Calligraphic letters
\newcommand{\mH}{\mathcal{H}}
\newcommand{\mJ}{\mathcal{J}}
\newcommand{\mK}{\mathcal{K}}
\newcommand{\mW}{\mathcal{W}}

% Operators
% Letters
\newcommand{\hA}{\hat{A}}
\newcommand{\hD}{\hat{D}}
\newcommand{\hH}{\hat{H}}
\newcommand{\hU}{\hat{U}}
\newcommand{\hh}{\hat{h}}
\newcommand{\hr}{\hat{r}}

% Calligraphic letters
\newcommand{\hmH}{\hat{\mathcal{H}}}
\newcommand{\hmX}{\hat{\mathcal{X}}}

% Bold letters
\newcommand{\hbD}{\hat{\boldsymbol{D}}}
\newcommand{\hbe}{\hat{\boldsymbol{e}}}
\newcommand{\hbr}{\hat{\boldsymbol{r}}}

% Bold symbols
\newcommand{\hbmu}{\mkern2mu\hat{\mkern-2mu\boldsymbol{\mu}}}
\newcommand{\hbmX}{\mkern4mu\hat{\mkern-4mu\boldsymbol{\mathcal{X}}}}

\RequirePackage{amsmath}
\RequirePackage{mathtools}
\RequirePackage{amssymb}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%                            General mathematics                         %%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\eps}{\varepsilon}                              %    Variant epsilon
\newcommand{\vphi}{\varphi}                                 %        Variant phi

\newcommand{\Z}{\mathbb{Z}}                                 %           Integers
\newcommand{\R}{\mathbb{R}}                                 %       Real numbers
\newcommand{\Comp}{\mathbb{C}}                              %    Complex numbers
\newcommand{\wt}[1]{\widetilde{#1}}                         %         Wide tilde
\newcommand{\conj}[1]{{#1}^*}                               %  Complex conjugate
%\newcommand{\conj}[1]{\overline{#1}}                       %  Complex conjugate
\newcommand{\tens}{\otimes}                                 %     Tensor product

\DeclareMathOperator\Ord{\mathcal{O}}                       %        Big-O order
\DeclareMathOperator{\Real}{Re}                             %         Real part 
\DeclareMathOperator{\Imag}{Im}                             %         Imag part

\newcommand{\definedas}{\coloneq}

\DeclareMathOperator{\vecspan}{span}

% Derivatives credit: https://tex.stackexchange.com/questions/29179/
\newcommand{\der}[2][]{\frac{d#1}{d#2}}
\newcommand{\pder}[2][]{\frac{\partial#1}{\partial#2}}
\newcommand{\fder}[2][]{\frac{\delta#1}{\delta#2}}

\newcommand{\grad}{\nabla}                                  %           Gradient
\newcommand{\lap}{\nabla^2}                                 %          Laplacian

\DeclarePairedDelimiter\abs{\lvert}{\rvert}                 %                |x|
\DeclarePairedDelimiter\norm{\lVert}{\rVert}                %              ||x||
\DeclarePairedDelimiter\comm{[}{]}                          %          commutator
\DeclarePairedDelimiter\acomm{\{}{\}}                       %      anticommutator

\DeclareMathOperator{\erf}{erf}                             %     Error function
\DeclareMathOperator{\erfc}{erfc}                           %  Complementary erf
\DeclareMathOperator{\FT}{\mathcal{F}}                      %  Fourier transform

% I can't be bothered to remember whether trace command is uppercase or not
\DeclareMathOperator{\tr}{Tr}                               %              Trace
\DeclareMathOperator{\Tr}{Tr}                               %              Trace
\DeclareMathOperator{\diag}{diag}                           %           Diagonal

% Floating point
\DeclareMathOperator{\FPD}{FP64}                            %   double precision
\DeclareMathOperator{\FPT}{TF32}                            %        tensorfloat
\DeclareMathOperator{\FPS}{FP32}                            %   single precision

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%                        General quantum mechanics                       %%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\newcommand{\Hilb}{\mathscr{H}}                             %      Hilbert space
\newcommand{\Hilb}{\mathcal{H}}                             %      Hilbert space
\newcommand{\Op}[1]{\hat{#1}}                               %           Operator
%\newcommand{\Op}[1]{#1}                                    %    No hat operator
\newcommand{\Ham}{\Op{H}}                                   %        Hamiltonian
\newcommand{\Id}{\Op{I}}                                    %  Identity operator
\newcommand{\Channel}{\mathcal{E}}                          %    Quantum channel
\newcommand{\Liouville}{\mathcal{L}}                        %        Liouvillian
\newcommand{\Redfield}{\mathcal{R}}                         %  Redfield operator

\newcommand{\up}{\uparrow}                                  %            Spin up
\newcommand{\dw}{\downarrow}                                %          Spin down

% Creation and annihilation operators with custom letters
\newcommand{\cre}[1]{\Op{#1}^\dagger}                       %           Creation
\newcommand{\ann}[1]{\Op{#1}}                               %       Annihilation

\newcommand{\adag}{\Op{a}^\dagger}                          %           Cre. a^+
\newcommand{\ades}{\Op{a}}                                  %             Ann. a
\newcommand{\bdag}{\Op{b}^\dagger}                          %           Cre. b^+
\newcommand{\bdes}{\Op{b}}                                  %             Ann. b
\newcommand{\cdag}{\Op{c}^\dagger}                          %           Cre. c^+
\newcommand{\cdes}{\Op{c}}                                  %             Ann. c

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%                            Abbreviations                               %%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\occ}{\ensuremath{\text{occ}}}                  %  Occupied orbitals
\newcommand{\vir}{\ensuremath{\text{vir}}}                  %   Virtual orbitals
\newcommand{\ext}{\ensuremath{\text{ext}}}                  %           External
\newcommand{\inv}{\ensuremath{\text{inv}}}                  %            Inverse
\newcommand{\scf}{\ensuremath{\text{scf}}}                  %   Self-cons. field
\newcommand{\Har}{\ensuremath{\text{H}}}                    %            Hartree
\newcommand{\kin}{\ensuremath{\text{T}}}                    %            kinetic
\newcommand{\aux}{\ensuremath{\text{aux}}}                  %          Auxiliary
\newcommand{\elec}{\ensuremath{\text{e}}}                   %           Electron
\newcommand{\phon}{\ensuremath{\text{pn}}}                  %             Phonon
\newcommand{\phot}{\ensuremath{\text{ph}}}                  %             Photon
\newcommand{\hc}{\ensuremath{\text{h.c.}}}                  %    Herm. conjugate
\newcommand{\emb}{\ensuremath{\text{emb}}}                  %          Embedding
\newcommand{\HF}{\text{HF}}                                 %       Hartree-Fock
\newcommand{\PC}{\text{PC}}                                 %     Primitive cell
\newcommand{\SC}{\text{SC}}                                 %          Supercell
\newcommand{\BZ}{\text{BZ}}                                 %     Brillouin zone
\newcommand{\prev}{\text{prev}}                             %    Prev. iteration
\newcommand{\mc}{\text{MC}}                                 %        Monte Carlo
\newcommand{\MC}{\text{MC}}                                 %        Monte Carlo
\newcommand{\QMC}{\text{QMC}}                               %          Quantum "
\newcommand{\qmc}{\text{QMC}}                               %          Quantum "
\newcommand{\AFQMC}{\text{AFQMC}}                           %  Auxiliary-field "
\newcommand{\afqmc}{\text{AFQMC}}                           %  Auxiliary-field "
\newcommand{\AO}{\text{AO}}                                 %    Atomic orbitals
\newcommand{\trial}{\text{T}}                               %        (QMC) trial
\newcommand{\Trial}{\text{T}}                               %        (QMC) trial
\newcommand{\inter}{\text{int}}                             %        Interaction
\newcommand{\hprec}{\text{h}}                               %     High precision
\newcommand{\lprec}{\text{l}}                               %      Low precision
\newcommand{\hlprec}{\text{hl}}                             %     Both precision
\newcommand{\dfp}{\text{FP64}}                              %               FP64
\newcommand{\sfp}{\text{FP32}}                              %               FP32
\newcommand{\tfp}{\text{TF32}}                              %               TF32
\newcommand{\tay}{\text{Taylor}}                            %       Taylor order

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%                            Dirac notation                              %%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\DeclarePairedDelimiter\bra{\langle}{\rvert}               %                 <a|
\DeclarePairedDelimiter\ket{\lvert}{\rangle}               %                 |a>
\DeclarePairedDelimiterX\ip[1]{\langle}{\rangle}
  {#1 \delimsize| #1}                                      %               <a|a>
\DeclarePairedDelimiterX\op[1]{\lvert}{\rvert} 
  {#1 \delimsize\rangle\!\delimsize\langle #1}             %              |a><a|
\DeclarePairedDelimiterX\braket[2]{\langle}{\rangle}
  {#1 \delimsize| #2}                                      %               <a|b>
\DeclarePairedDelimiterX\ketbra[2]{\lvert}{\rvert} 
  {#1 \delimsize\rangle\!\delimsize\langle #2}             %              |a><b|
\DeclarePairedDelimiter\evo{\langle}{\rangle}              %                 <O>
\DeclarePairedDelimiterX\ev[2]{\langle}{\rangle}
  {#2 \delimsize| #1 \delimsize| #2}                       %             <a|O|a>
\DeclarePairedDelimiterX\mel[3]{\langle}{\rangle}
  {#1 \delimsize| #2 \delimsize| #3}                       %             <a|O|b>

\DeclarePairedDelimiter\normalord{:}{:}                    % Normal ordering
